Entanglement-Assisted Quantum Error-Correcting Codes with Imperfect Ebits

The scheme of entanglement-assisted quantum error-correcting (EAQEC) codes assumes that the ebits of the receiver are error-free. In practical situations, errors on these ebits are unavoidable, which diminishes the error-correcting ability of these codes. We consider two different versions of this problem. We first show that any (nondegenerate) standard stabilizer code can be transformed into an EAQEC code that can correct errors on the qubits of both sender and receiver. These EAQEC codes are equivalent to standard stabilizer codes, and hence the decoding techniques of standard stabilizer codes can be applied. Several EAQEC codes of this type are found to be optimal. In a second scheme, the receiver uses a standard stabilizer code to protect the ebits, which we call a "combination code." The performances of different quantum codes are compared in terms of the channel fidelity over the depolarizing channel. We give a formula for the channel fidelity over the depolarizing channel (or any Pauli error channel), and show that it can be efficiently approximated by a Monte Carlo calculation. Finally, we discuss the tradeoff between performing extra entanglement distillation and applying an EAQEC code with imperfect ebits.

==> LinearProgramming.tex <==
\section{Linear Programming Bound for Non-Maximal-Entanglement Quantum Codes}

%\subsection{The Linear Programming Bounds for EAQEC Codes with Maximal Entanglement}

Quantum MacWilliams identity is proved by Shor and Laflamme \cite{SL96}
 and its stabilizer code version is proved by Gottesman \cite{Got97}.
Lai, Brun, and Wilde proved the EAQEC version \cite{LBW10}.
These identities describe a relation between the weight enumerators of a group $\mathcal{S}$ and its dual,
which is the normalizer group $\mathcal{N}(\mathcal{S})$.
Suppose that $A(z)$ and $B(z)$ are the weight enumerators of $\mathcal{S}$ and $\mathcal{N}(\mathcal{S})$, respectively.
It turns out that these identities have the same form as the classical linear quaternary codes:
\begin{align*}
B(z)=\frac{1}{|\mathcal{S}|}(1+3z)^n A\left(\frac{1-z}{1+3z}\right),
\end{align*}
or
\begin{align*}
B_w=& \frac{1}{|\mathcal{S}|} \sum_{w'=0}^n P_w(w',n) A_{w'}, \label{eq:QuantumMacWilliamsEAQEC}
\end{align*}
for $w=0,\cdots, n$,
where
\[
P_w(w',n)= \sum_{u=0}^{w}(-1)^u 3^{w-u} {w'\choose u}{n-w'\choose w-u}
\]
is the Krawtchouk polynomial \cite{MS77}.

For an $[[n,k,d;c]]$ EAQEC code in general, we have a symplectic subgroup $\mathcal{S}_S$ and an isotropic subgroup $\mathcal{S}_I$ of the stabilizer group,  and a logical subgroup $\mathcal{L}$,
where $\mathcal{L}\times \mathcal{S}_I$ and $\mathcal{S}_S\times \mathcal{S}_I$  are dual to each other.
Please refer to \cite{BDM06,LB10,LBW10} for basics of EAQECCs.
In the case of maximal-entanglement quantum codes ($c=n-k$), we have $\mathcal{S}_I=\emptyset$, and
 $\mathcal{S}_S$ and $\mathcal{L}$  are dual to each other.
In the case of standard stabilizer codes ($c=0$), we have $\mathcal{S}_S=\emptyset$, and
 $\mathcal{S}_I$ and $\mathcal{L}\times \mathcal{S}_I$  are dual to each other.


The minimum distance of an EAQEC code (or  a standard stabilizer code) is
the minimum weight of any element in $(\mathcal{L}\times \mathcal{S}_I) \backslash \mathcal{S}_I$.
Suppose the weight enumerators of   $\mathcal{S}_S\times \mathcal{S}_I$ and $\mathcal{L}\times \mathcal{S}_I$ are $A(z)$ and $B(z)$, respectively.
For $c=0$ or $c=n-r$, the minimum distance  can be determined from the coefficients of the weight enumerators $A(z)$ and $B(z)$, which are constrained by the MacWilliams identities.
Thus the linear programming techniques can be applied to find an upper bound on the minimum distance of these quantum codes.
This is called the linear programming bound.
However,  the linear programming bound for the case $0<c<n-k$ is unknown.
We will proceed to a solution to this problem in this article.

%The minimum distance of an EAQEC code is the minimum weight of any element in $\mathcal{L}\times \mathcal{S}_I\backslash \mathcal{S}_I$.






Now we consider the case $0<c<n-k$ and $\mathcal{S}_I\neq \emptyset$, $\mathcal{S}_S\neq \emptyset$.
Observe that
\[
    \mathcal{N}(\mathcal{S}_I)= \mathcal{L}\times \mathcal{S}_S\times  \mathcal{S}_I.
\]
If we view the group $( \mathcal{L}\times \mathcal{S}_S)$ as a logical group of a standard stabilizer code with a stabilizer group $\mathcal{S}_I$,
this is just the dual relation of the standard stabilizer codes.
Let  the weight enumerator of $\mathcal{S}_I$ be $C(z)$ and the weight enumerator of $\mathcal{L}\times \mathcal{S}_S\times  \mathcal{S}_I$ be $D(z)$.
Then $C(z)$ and $D(z)$ are related by the MacWilliams identity for standard stabilizer codes.
The minimum distance of the EAQEC code is the minimum nonzero integer $w$ such that $A_w-C_w>0$.
With constraints on $A_w$'s and  $C_w$'s, we can find the linear programming bound on the minimum distance.
To sum up, we have the following constraints:
{
%\small
%\footnotesize
%\scriptsize
\begin{align*}
&A_0=B_0=C_0=D_0=1;\\
&A_w\geq 0, B_w \geq 0, C_w\geq 0, D_w \geq 0, \mbox{ for $w=1, \cdots, n$};\\
&A_w\leq |\mathcal{S}_S\times \mathcal{S}_I|, B_w \leq |\mathcal{L}\times \mathcal{S}_I|, \mbox{ for $w=1, \cdots, n$};\\
&C_w\leq |\mathcal{S}_I|, D_w \leq | \mathcal{L}\times \mathcal{S_S}\times\mathcal{S}_I|,\mbox{ for $w=1, \cdots, n$};\\
&D_w\geq A_w, D_w\geq B_w, D_w\geq C_w,  \mbox{ for $w=1, \cdots, n$};\\
&A_w \geq C_w, B_w \geq C_w, \mbox{ for $w=1, \cdots, n$};\\
%\end{align*}
%\begin{align*}
&\sum_{w=0}^n A_w= |\mathcal{S}_S\times \mathcal{S}_I|, \sum_{w=0}^n B_w =|\mathcal{L}\times \mathcal{S}_I|,\\
&\sum_{w=0}^n C_w= |\mathcal{S}_I|, \sum_{w=0}^n D_w =|\mathcal{L}\times  \mathcal{S_S}\times \mathcal{S}_I|;\\
&B_w=\frac{1}{|\mathcal{S}_S\times \mathcal{S}_I|} \sum_{w'=0}^n P_w(w',n) A_{w'},
\ \mbox{ for $w=0, \cdots, n$};\\
&D_w=\frac{1}{| \mathcal{S}_I|} \sum_{w'=0}^n  P_w(w',n) C_{w'},
\ \mbox{ for $w=0, \cdots, n$};\\
%\end{align*}
%\begin{align*}
&B_w=C_w,   \mbox{ for $w=1, \cdots, d-1$};\\
%&B_w\geq C_w,   \mbox{ for $w=d, d+1 \cdots, n$};
\end{align*}
}

There is no linear function to be optimized in this coding problem.
If we cannot find any solutions to the integer programming problem with the above
constraints for a certain $d$, this result implies that there is no $[[n,k,d; c]]$ EAQEC code.
If
$d^*$ is the smallest of such $d$'s, then $d^*-1$ is an upper bound
on the minimum distance of an $[[n,k,d;c]]$ EAQEC code. This is
the linear programming bound for EAQEC codes with $0<c<n-k$.
If we change the constraints
\begin{align*}
&B_w=C_w,   \mbox{ for $w=1, \cdots, d-1$},
%&B_w\geq C_w,  \mbox{ for $w=d, d+1 \cdots, n$};
\end{align*}
with
\begin{align*}
&A_w=C_w,   \mbox{ for $w=1, \cdots, d-1$},
%&A_w\geq C_w,   \mbox{ for $w=d, d+1 \cdots, n$};
\end{align*}
this gives the constraints of the linear programming bound on the minimum distance of
the $[[n,c,d;k]]$ dual code.

\be
 The linear programming bound of the $[[7,1;4]]$ code is $d\leq 6$, which is the same as the singleton bound.
Hence the $[[7,1,5;4]]$ EA quantum code from the encoding optimization algorithm in Example 4 of \cite{LB10} does not achieve the linear programming bound.
It follows that the $[[7,1,5;5]]$ does not achieve the upper bound either.
\ee

\be
The linear programming bound of the $[[8,3;3]]$ code is $d\leq 4$, which improves the singleton bound: $d\leq 5$.
Hence the $[[8,3,4;3]]$ EA quantum code from the encoding optimization algorithm  in Example 8 of \cite{LB10} is optimal.
On the other hand,
the linear programming bound of the $[[8,3;4]]$ code is $d\leq 5$, which is the same as the singleton bound.
Hence the $[[8,3,4;4]]$ EA quantum code does not achieve the upper bound.
\ee

\be
The linear programming bounds of $[[9,1;c]]$ codes for $c=3,4,5$  are $d\leq 8$; however, the singleton bound is $d\leq 6$, $d\leq 7$, and $d\leq 7$, respectively.
%The linear programming bound of a $[[9,1;3]]$ code is $d\leq 8$; however, the singleton bound is $d\leq 6$.
\ee

From these three examples, the linear programming bound might be better or worse than the singleton bound when $0<c<n-k$.

\section{Generalization of the Encoding Optimization Algorithm}
We can extend the encoding optimization algorithm from the form in \cite{LB10}, by starting the optimization from a good EAQEC code and adding additional entanglement.
From a given $[[n,k,d;c ]]$ code,
we can change any subsets of the $n-k-c$ ancilla qubits with ebits and then apply a similar encoding optimization algorithm.
From a given ``good'' $[[n,k,d_1;c ]]$ code, we obtain an optimized $[[n,k,d';n-k ]]$ code much faster than using the original optimization over an $[[n,k,d_2]]$ code.
Since we begin with a ``good"  $[[n,k,d_1;c ]]$ code,  the optimized $[[n,k,d';n-k ]]$ code is expected to approach the upper bound. %on the minimum distance.
Such a ``good" code can be obtained from the construction in \cite{BDM06}, using optimal classical quaternary codes.

\section{Self-Dual EAQEC Codes}




Consider the  possibility of a ``self-dual code'' $[[n, n/2,d; n/2]]$ for $n$
even, such that the dual code is also an $[[n,n/2,d; n/2]]$ code with the same
weight enumerators. That is, $B(z)=A(z)$.
We conjecture that such self-dual codes exist. % with the minimum distance $d= \frac{n}{2}$.
If so, the two groups $\mathcal{S}_S$ and $\mathcal{L}$ may be equivalent up to a permutation on the qubits.

Shadow enumerators, designed for self-dual codes, give additional constraints on the weight
enumerator of a stabilizer code.




\subsection{Shadow Enumerator}
The shadow $Sh(\mathcal{S})$ of a group $\mathcal{S}$ is defined as the set of $E\in \mathcal{G}^n$ satisfying that
\[
E\odot M =wt(M) \mod 2,
\]
for all $M\in \mathcal{S}$ \cite{Rains96}.
Then the  shadow $Sh(\mathcal{S})$ is just  $\mathcal{N}(\mathcal{S}_e)-\mathcal{N}(\mathcal{S})$,
where $\mathcal{S}_e$ is the subset of $\mathcal{S}$ of even weight operators.
Let $S(z)$ be the weight enumerator of $Sh(\mathcal{S})$.
Rains proved a relation between the shadow enumerator and the weight enumerator of a quantum code \cite{Rains96}.
For stabilizer codes, $|\mathcal{S}_e|=\frac{1}{2}|\mathcal{S}|$. Then
\begin{align*}
S(z)= B_e(z)-B(z)= \frac{1}{|\mathcal{S}|}(1+3z)^n A\left( \frac{z-1}{1+3z}\right),
\end{align*}
where $ B_e(z), B(z)$ are the weight enumerators of $\mathcal{N}(\mathcal{S}_e)$ and $\mathcal{N}(\mathcal{S})$, respectively.

However, in the case of EAQECCs, the situation is different.
Suppose $S(z)$ is the shadow enumerator of $\mathcal{S}'= \mathcal{S}_S \cup \mathcal{S}_I$ of an EAQEC code with a weight enumerator $A(z)$.
We have
\[
S(z)=B_e(z)-B(z).
\]
In general, we know nothing about $B_e(z)$.

$****************$To be finished$*************************$
%We have the the same relation in the case of EAQECCs.
\bt
Suppose $S(z)$ is the shadow enumerator of $\mathcal{S}'= \mathcal{S}_S \cup \mathcal{S}_I$ of an EAQEC code with a weight enumerator $A(z)$.
Then
\begin{align*}
S(z)= \frac{1}{|\mathcal{S}'|}(1+3z)^n A\left( \frac{z-1}{1+3z}\right).
\end{align*}
\et
while Gottesman gave the proof for quantum stabilizer codes \cite{Got97}.
The proof for general stabilizer codes by Gottesman applies to the case of EAQECCs.
Therefore, this relation yields new constraints on the coefficients of the weight enumerator of an EAQEC code,
which makes the linear programming bound tighter.

% However, there is no general form in the case of EAQEC codes.


\section{Nonexistence of EAQEC Codes by Linear Programming Bounds}
We proved the non-existence of $[[n,1,n;n-1]]$ or $[[n,n-1,2;1]]$ codes for $n$ even,
which  decreases the upper bound predicted by the linear programming bound for $k=1$ and $n$ even.



\section{Upper and Lower Bounds on the Minimum Distance of EAQEC Codes}
Similar to Table 1 in \cite{LBW10}, we can construct tables of upper and lower bounds on the minimum distance of EAQEC codes for each $c$.

